Sequential Covariance Fitting for InSAR Phase Linking

Traditional Phase-Linking (PL) algorithms are known for their high cost, especially with the huge volume of Synthetic Aperture Radar (SAR) images generated by Sentinel-1 SAR missions. Recently, a COvariance Fitting Interferometric Phase Linking (COFI-PL) approach has been proposed, which can be seen as a generic framework for existing PL methods. Although this method is less computationally expensive than traditional PL approaches, COFI-PL exploits the entire covariance matrix, which poses a challenge with the increasing time series of SAR images. However, COFI-PL, like traditional PL approaches, cannot accommodate the efficient inclusion of newly acquired SAR images. This paper overcomes this drawback by introducing a sequential integration of a block of newly acquired SAR images. Specifically, we propose a method for effectively addressing optimization problems associated with phase-only complex vectors on the torus based on the Majorization-Minimization framework.

==> plus.tex <==
\subsection{\acl{KL} divergence}
\label{subsection:KL_seq}

\noindent
This section is divided into two parts: the first part covers the cost functions, followed by the various solution methods.

\subsubsection{Cost functions}

\noindent
In this section, we provide the cost function for each distance and various covariance matrix plug-ins.

    \paragraph{\ac{SCM} / \ac{PO}}
    
    \noindent
    Using the objective function in (\ref{cost_fct_KL}) and the block structure of the covariance and coherence matrix respectively in (\ref{bloc_cov}), (\ref{bloc_coh}) the \ac{KL} divergence can be written as follow
    \begin{proposition}
    Cost function for \ac{KL} divergence with the \ac{SCM} / \ac{PO} as a plug-in
    \begin{align}
    \label{eq:cost_fct_KL_unstructured_cov}
        &f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta})  = \mathbf{w}_{\theta}^H \left( \mathbf{F}^{-1} \circ \mathbf{\Sigma} \right) \mathbf{w}_{\theta}  \\
        &\qquad + \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ  \mathbf{V}^H \right)\mathbf{\Bar{w}}_{\theta} \notag \\
        &\qquad + \mathbf{\Bar{w}}_{\theta}^H \left( \left( - \mathbf{D}^{-1} \mathbf{A} \mathbf{\Psi}^{-1}\right)\circ  \mathbf{V} \right) \mathbf{w}_{\theta} \notag \\
        &+ \mathbf{\Bar{w}}_{\theta}^H \left( \mathbf{D}^{-1} \circ \mathbf{Z}\right) \mathbf{\Bar{w}}_{\theta} \notag
    \end{align}
    \end{proposition}
    where 
    \begin{itemize}
        \item[-] $\mathbf{F} = \mathbf{\Psi} - \mathbf{A}^T \mathbf{B}^{-1}\mathbf{A}$
        \item[-] $\mathbf{D} = \mathbf{B} - \mathbf{A}\mathbf{\Psi}^{-1}\mathbf{A}^T$
    \end{itemize}
    Calculation details are provided in Appendix \ref{app_CF_KL_unstruct}
    
    \paragraph{Shrinkage to identity}
    
    The block structure of the shrinkage to identity regularization of a plug-in of the covariance matrix (\ref{cov_mat_shrink}) can be represented as follow
    \noindent\resizebox{\columnwidth}{!}{
    \begin{minipage}{\columnwidth}
    \begin{align}
        \mathbf{\widetilde{\Sigma}} &= \left( \begin{array}{cc}
            \beta \mathbf{\Sigma} + (1 - \beta) \frac{\text{tr}(\mathbf{\widetilde{\Sigma}})}{l} \mathbf{I}_p & \beta \mathbf{V}^H \\
            \beta \mathbf{V} & \beta \mathbf{Z} + (1 - \beta) \frac{\text{tr}(\mathbf{\widetilde{\Sigma}})}{l} \mathbf{I}_k \\
        \end{array} \right)
    \label{bloc_shrink}
    \end{align}
    \end{minipage}
    }
    given that the estimator can be either the \ac{SCM} or \ac{PO}. The structure in (\ref{bloc_shrink}) make minor differences in the form of the cost function in (\ref{eq:cost_fct_KL_unstructured_cov}), and then will have the following form
    \begin{proposition}
    Cost function for \ac{KL} divergence with a shrinked estimator to identity
    \begin{align}
        \label{cost_fct_KL_shrink}
        &f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta}) = \mathbf{w}_{\theta}^H \left(\mathbf{F}^{-1} \circ \mathbf{\hat{\Sigma}} \right) \mathbf{w}_{\theta} \notag \\
        &\quad + \beta \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ  \mathbf{V}^H \right)\mathbf{\Bar{w}}_{\theta} \notag \\
        &\quad + \beta \mathbf{\Bar{w}}_{\theta}^H \left( \left( - \mathbf{D}^{-1} \mathbf{A}\mathbf{\Psi}^{-1}\right)\circ  \mathbf{V} \right) \mathbf{w}_{\theta}  \notag \\
        &+ \mathbf{\Bar{w}}_{\theta}^H \left( \mathbf{D}^{-1} \circ \mathbf{Y} \right) \mathbf{\Bar{w}}_{\theta} 
    \end{align}
    where 
    \begin{itemize}
        \item[-] $\mathbf{\hat{\Sigma}} = \beta \mathbf{\Sigma} + (1 - \beta) \frac{\text{tr}(\mathbf{\widetilde{\Sigma}})}{l} \mathbf{I}_p $
        \item[-] $\mathbf{Y} = \beta \mathbf{Z} + (1 - \beta) \frac{\text{tr}(\mathbf{\widetilde{\Sigma}})}{l} \mathbf{I}_k$
    \end{itemize}
    \end{proposition}
    Further details on the cost function computation are given in Appendix \ref{app_CF_KL_shrink}
    
    \paragraph{Covariance matrix tapering}
    
    The tapering matrix with bandwidth $\textit{b}$ in eq. (\ref{tap}) can be partitioned as the following block structure 

    \begin{align}
        \label{bloc_tapering}
        \mathbf{\widetilde{W}}(b)
        &= \left( \begin{array}{c}
            \begin{tabular}{ccc}
                $\mathbf{W}$ & $\mathbf{U}^T$ \\
                     $\mathbf{U}$      &  $\mathbf{T}$ \\
            \end{tabular}
        \end{array} \right)
    \end{align}
    
    Then the tapered covariance matrix will have the following structure
    \begin{align}
        \mathbf{\widetilde{\Sigma}}(b) &=  \mathbf{W}(b) \circ \mathbf{\Hat{\Sigma}} \\
        &= \left( \begin{array}{c}
            \begin{tabular}{cc}
                $\mathbf{W} \circ \mathbf{\Sigma}$ & $\mathbf{U}^T \circ\mathbf{V}^H$ \\
                $\mathbf{U} \circ \mathbf{V}$      &  $ \mathbf{T} \circ \mathbf{Z}$ \\
            \end{tabular}
        \end{array} \right)
         \label{tapered_bloc_cov}
    \end{align}
    
    The corresponding cost function is presented as follow
    
    \begin{proposition}
    Cost function for \ac{KL} divergence with a tapered estimator
    %\noindent\resizebox{\columnwidth}{!}{
    %\begin{minipage}{\columnwidth}
    \begin{align}
        f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta}) &= \mathbf{w}_{\theta}^H \left( \mathbf{F}^{-1} \circ ( \mathbf{W} \circ \mathbf{\Sigma}) \right) \mathbf{w}_{\theta} \notag \\
        &+ \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ  (\mathbf{U}^T \circ\mathbf{V}^H) \right)\mathbf{\Bar{w}}_{\theta} \notag \\
        &+ \mathbf{\Bar{w}}_{\theta}^H \left( \left( - \mathbf{D}^{-1} \mathbf{A} \mathbf{\Psi}^{-1}\right)\circ  (\mathbf{U} \circ \mathbf{V}) \right) \mathbf{w}_{\theta} \notag \\
        &+ \mathbf{\Bar{w}}_{\theta}^H \left( \mathbf{D}^{-1} \circ(\mathbf{T} \circ \mathbf{Z}) \right) \mathbf{\Bar{w}}_{\theta}
        \label{cost_fct_KL_tap}
    \end{align}
    %\end{minipage}
    %}
    \end{proposition}
More details on the cost function computation are given in Appendix \ref{app_CF_KL_tap}.




% MM KL
    \paragraph{\ac{MM} algorithm}
    
    For each  case of the generic cost function for the \ac{KL} divergence \ref{prop:prop_CF_KL} and after a few calculations steps, it corresponds to the convex quadratic form in Lemma \ref{lemma1}. As same as the cost function, we present a generic form for the surrogate function that majorizes the corresponding cost function \ref{prop:prop_CF_KL} 

    \begin{proposition}
    Majorization function for the \ac{KL} divergence
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) &= - \textit{Re} \left( 2 \mathbf{\Bar{w}}_{\theta}^H  \left(  \left[ \left( \mathbf{D}^{-1} \mathbf{A}\mathbf{\Psi}^{-1} \right) \circ \mathbf{V} \right] \mathbf{w}_{\theta} \right. \right. \notag\\
        &\left. \left. - \left[ \left( \mathbf{D}^{-1} \circ \mathbf{Z} \right) - \lambda_{\text{max}} \mathbf{I} \right] \mathbf{\Bar{w}}_{\theta}^{(t)} \right) \right)
    \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_KL_unstruct}.
    
    \begin{proposition}
    Majorization function for the \ac{KL} divergence along with the shrinking to identity regularization
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) &= - \textit{Re}\left( \mathbf{\Bar{w}}_{\theta}^H  2 \left[ \beta \left( \left( \mathbf{D}^{-1} \mathbf{A}\mathbf{\Psi}^{-1}\right)\circ  \mathbf{V} \right) \mathbf{w}_{\theta} \right. \right. \notag \\
        &\left. -  \left. \left[ \left( \mathbf{D}^{-1} \circ \mathbf{Y} \right) - \lambda_{max} \mathbf{I}_k \right] \mathbf{\Bar{w}}_{\theta}^{(t)}   \right] \right)
    \end{align}
    \end{proposition}
    More details can be found in Appendix \ref{app_MM_KL_shrink}.
    
    \begin{proposition}
        Majorization function for the \ac{KL} divergence along with the covariance matrix tapering regularization
        \begin{align}
            g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) &= - \textit{Re} \left( 2 \mathbf{\Bar{w}}_{\theta}^H  \left(  \left[ \left( \mathbf{D}^{-1} \mathbf{A}\mathbf{\Psi}^{-1} \right) \circ (\mathbf{U} \circ \mathbf{V}) \right] \mathbf{w}_{\theta} \right. \right. \notag\\
            &\left. \left. - \left[ \left( \mathbf{D}^{-1} \circ (\mathbf{T} \circ \mathbf{Z}) \right) - \lambda_{\text{max}} \mathbf{I} \right] \mathbf{\Bar{w}}_{\theta}^{(t)} \right) \right)
        \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_KL_tap}.
    %For (\ref{cost_fct_KL_shrink}), details can be found in Appendix \ref{app_MM_KL_struct}. 
    

    
    The equivalent optimization to (\ref{eq:prob_optim_fitting_online}) problem will be then
    \begin{equation}
    %\label{eq:phaselinking}
        \begin{array}{c l}
        \underset{\mathbf{\Bar{w}}_{\theta} \in \mathbb{T}_k}{\rm minimize}
        & 
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)})
        \end{array}
    \end{equation}
    and is solved using Lemma \ref{lemma2}


    \begin{algorithm}[H]
    \caption{\ac{MM} for \ac{KL} divergence with \ac{SCM} / \ac{PO} plug-in}
    \begin{algorithmic}[1]
        \State \textbf{Input}: $\mathbf{\tilde{\Sigma}} \in \mathbb{C}^l$, $\mathbf{w}_{\theta}^{(0)} \in \mathbb{T}_l$
        \State Compute : $\mathbf{M} = 2 (\mathbf{D}^{-1} \circ \mathbf{Z})$ 
        \State Compute $ \mathbf{N} = 2  \left[ \left( \mathbf{D}^{-1} \mathbf{A}\mathbf{\Psi}^{-1} \right) \circ \mathbf{V}\right] \mathbf{w}_{\theta} $
        \Repeat
            \State Compute $\mathbf{\bar{w}}_{\theta}^{(t)} = \mathbf{N} - (\mathbf{M} - \lambda_{max}^{\mathbf{M}} \mathbf{I}) w^{(t)}$
            \State Update of $\mathbf{\bar{w}}_{\theta}^{(t)} = \phi_{\mathbb{T}}\{ \bar{\mathbf{w}}_{\theta}^{(t)} \} $ 
            \State $t = t + 1$
        \Until{convergence}
        \State \textbf{Output}: $\hat{\mathbf{w}}_{\theta} = \mathbf{w}_{end} \in \mathbb{T}_k$
    \end{algorithmic}
    \end{algorithm}

    % RGD KL
        
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with \ac{SCM} / \ac{PO} plug-in
    \begin{align}
        \textit{grad} f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}} &= \left( 2 \left[ \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ  \mathbf{V}^H \right) \right. \right. \notag \\
        &\left. \left. +  \mathbf{\Bar{w}}_{\theta}^H  \left( \mathbf{D}^{-1} \circ \mathbf{Z}\right) \right] \right)^H
        \label{grad_KL_unstruct}
    \end{align}
    \end{proposition}
    
    More details about the calculations can be found in Appendix \ref{app_RGD_KL_unstruct}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with shrinking to identity regularization
    \begin{align}
        \textit{grad} f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}} &= \left( 2 \left[ \beta \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ  \mathbf{V}^H \right)  \right. \right. \notag \\
        &\left. \left. + \mathbf{\Bar{w}}_{\theta}^H \left( \mathbf{D}^{-1} \circ \mathbf{Y}  \right) \right] \right)^H
        \label{grad_KL_shrink}
    \end{align}
    \end{proposition}
    
    Further details about the calculations can be found in Appendix \ref{app_RGD_KL_shrink}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with tapered covariance matrix
    \begin{align}
        \textit{grad} f^{\text{KL}}_{\mathbf{\widetilde{\Sigma}}} &= \left( 2 \left[ \mathbf{w}_{\theta}^H \left( \left( - \mathbf{\Psi}^{-1} \mathbf{A}^T  \mathbf{D}^{-1} \right) \circ (\mathbf{U}^T \circ\mathbf{V}^H) \right) \right. \right. \notag \\
        &\left. \left. +  \mathbf{\Bar{w}}_{\theta}^H  \left( \mathbf{D}^{-1} \circ (\mathbf{T} \circ \mathbf{Z}) \right) \right] \right)^H
        \label{grad_KL_tap}
    \end{align}
    \end{proposition}
    
    Additional details about the calculations can be found in Appendix \ref{app_RGD_KL_tap}.
    
    %Further details on calculations can be found in Appendix \ref{app_RGD_KL}. 
    %\begin{figure}
        %\centering
        %\input{tikz/manifold}
        %\caption{\\ac{RGD} illustration on a unit complex cercle}
        %\label{fig:manifold}
    %\end{figure}
    \begin{algorithm}[H]
    \caption{\ac{RGD} algorithm for \ac{KL} divergence with an unstructured plug-in}
    \begin{algorithmic}
        \State \textbf{Input}: Objective function \( f \) (eq. \ref{eq:cost_fct_KL_unstructured_cov}), starting point \( \mathbf{\bar{w}}_{\theta}^{(0)} \)
        \Repeat
            \State Compute euclidean gradient with (\ref{grad_KL_unstruct})
            \State Compute Riemannian gradient with (\ref{inner_product})
            \State Set direction \( \mathbf{\xi}^{(t)} = - \alpha \eta^{(t)} \)
            \State Update \( \mathbf{\bar{w}}_{\theta}^{(t)} = \mathcal{R}_{\mathbf{w}_{\theta}^{(t)}}(\mathbf{\xi}^{(t)}) \)
        \Until{convergence}
        \State \textbf{Output}: \( \hat{\mathbf{w}}_{\theta} = \mathbf{\bar{w}}_{\text{end}} \in \mathbb{T}_k \)
    \end{algorithmic}
\end{algorithm}

%%% Frob
Similar to the \ac{KL} divergence, this section is also divided into two parts: the first part addresses the cost functions, followed by the various solution methods.

\subsubsection{Cost functions}


    \paragraph{\ac{SCM}}
    
    Replacing the block structured covariance and coherence matrix (\ref{bloc_cov}), (\ref{bloc_coh}) respectively in the cost function \ref{cost_fct_LS} yield the following form
    \begin{proposition}
    Cost function for Frobenius norm with \ac{SCM} / \ac{PO}
    \begin{align}
        f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta})  &= - 2 \mathbf{w}_{\theta}^H (\mathbf{\Psi} \circ \mathbf{\Sigma}) \mathbf{w}_{\theta} - 2 \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) \mathbf{\Bar{w}}_{\theta}  \notag \\
        &- 2 \mathbf{\Bar{w}}_{\theta} ^H (\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} - 2 \mathbf{\Bar{w}}_{\theta} ^H (\mathbf{B} \circ \mathbf{Z}) \mathbf{\Bar{w}}_{\theta} 
        \label{cost_fct_bloc_Frob}
    \end{align}
    \end{proposition}
    
    Details for the cost function computation are given in Appendix \ref{app_CF_Frob_unstruct}.
    
    \paragraph{Shrinkage to identity}
    
    The block structure of the shrinkage to identity regularization of a plug-in of the covariance matrix in (\ref{bloc_shrink}) is used to obtain the corresponding cost function
    \begin{proposition}
    Cost function for Frobenius norm with a shrinked estimator to identity
    \begin{align}
        f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta}) &= - 2 \mathbf{w}_{\theta}^H (\mathbf{\Psi} \circ \mathbf{\hat{\Sigma}} ) \mathbf{w}_{\theta} \notag \\
        &- 2\beta \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) \mathbf{\Bar{w}}_{\theta} - 2\beta \mathbf{\Bar{w}}_{\theta}^H (\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} \notag \\
        &- 2 \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ \mathbf{Y}) \mathbf{\Bar{w}}_{\theta} 
        \label{cost_fct_bloc_Frob_shrink}
    \end{align}
    \end{proposition}
    
    Details for the cost function computation are given in Appendix \ref{app_CF_Frob_shrink}.
    
    \paragraph{Covariance matrix tapering}
    
    The tapered covariance matrix in (\ref{tapered_bloc_cov}) yield the following form of the cost function 
    
    \begin{proposition}
    Cost function for Frobenius norm with a tapering covariance matrix plug-in
    \begin{align}
        f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}}(\mathbf{\widetilde{w}}_{\theta})  &= - 2 \mathbf{w}_{\theta}^H (\mathbf{\Psi} \circ ( \mathbf{W} \circ \mathbf{\Sigma})) \mathbf{w}_{\theta} \notag \\
        &- 2 \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ (\mathbf{U}^T \circ\mathbf{V}^H) ) \mathbf{\Bar{w}}_{\theta}  \notag \\
        &- 2 \mathbf{\Bar{w}}_{\theta} ^H (\mathbf{A} \circ (\mathbf{U} \circ \mathbf{V}) ) \mathbf{w}_{\theta} \notag \\
        &- 2 \mathbf{\Bar{w}}_{\theta} ^H (\mathbf{B} \circ (\mathbf{T} \circ \mathbf{Z})) \mathbf{\Bar{w}}_{\theta} 
        \label{cost_fct_bloc_Frob_tap}
    \end{align}
    \end{proposition}

    Details for the cost function computation are given in Appendix \ref{app_CF_Frob_tap}.
\subsubsection{Resolution}

As for the \ac{KL} divergence case, the Frobenius norm case has two possible way to solve each problem.

    \paragraph{\ac{MM} algorithm}
    
    \begin{lemma}
    The concave quadratic form 
    \begin{equation}
        f : \mathbf{w}_{\theta} \longrightarrow - \mathbf{w}_{\theta}^H \mathbf{H} \mathbf{w}_{\theta}
    \end{equation}
    is majored, with equality at point $\mathbf{w}^{(t)}$ \cite{vu2024covariance},  by : 
    \begin{equation}
        g(\mathbf{w}_{\theta}|\mathbf{w}_{\theta}^{(t)}) = -\textit{Re}( \mathbf{w}^H \mathbf{H} \mathbf{w}_{\theta}^{(t)} )
    \end{equation}
    \label{lemma3}
    \end{lemma}
    Using Lemma \ref{lemma3}, each function of (\ref{cost_fct_bloc_Frob}),  (\ref{cost_fct_bloc_Frob_shrink}),  (\ref{cost_fct_bloc_Frob_tap}) can be majored by a function $g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)})$ which will provided in the next propositions.
    
    \begin{proposition}
    Majorization function for the Frobenius norm along with the \ac{SCM} / \ac{PO} plug-in 
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) = - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[(\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} +  (\mathbf{B} \circ \mathbf{Z}) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
    \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_Frob_unstruct}.
    
    \begin{proposition}
    Majorization function for the Frobenius norm along with the shrinking to identity regularization
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) = - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[\beta(\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} +  (\mathbf{B} \circ \mathbf{Y}) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
    \end{align}
    \end{proposition}
    More details can be found in Appendix \ref{app_MM_Frob_shrink}.
    
    \begin{proposition}
        Majorization function for the Frobenius norm along with the covariance matrix tapering regularization
        \begin{align}
            g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) &= - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[(\mathbf{A} \circ (\mathbf{U} \circ \mathbf{V}) ) \mathbf{w}_{\theta} \right. \right. \notag \\
            &\left. \left. +  (\mathbf{B} \circ (\mathbf{T} \circ \mathbf{Z})) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
        \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_Frob_tap}.
    
    \noindent
    Then the minimization problem can be solved using Lemma \ref{lemma2}.
    
    \begin{algorithm}[H]
    \caption{\\ac{MM} for Frobenius norm with an unstructured plug-in}
    \begin{algorithmic}[1]
        \State \textbf{Input}: $\mathbf{\tilde{\Sigma}} \in \mathbb{C}^l$, $\mathbf{w}_{\theta}^{(1)} \in \mathbb{T}_l$
        \State Compute  $\mathbf{M} = \mathbf{A} \circ \mathbf{V}$ 
        \State Compute  $\mathbf{N} = \mathbf{B} \circ \mathbf{Z}$ 
        \Repeat
            \State Compute $\mathbf{\bar{w}}^{(t)} = \mathbf{M} + \mathbf{N} w^{(t)}$
            \State Update of $ \mathbf{\bar{w}}_{\theta}^{(t)} = \phi_{\mathbb{T}}\{ \mathbf{\bar{w}}_{\theta}^{(t)} \} $ 
            \State $t = t + 1$
        \Until{convergence}
        \State \textbf{Output}: $\hat{\mathbf{w}}_{\theta} = \mathbf{\bar{w}}^{(\text{end})} \in \mathbb{T}_k$
    \end{algorithmic}
    \end{algorithm}

    \paragraph{Riemannian optimization}
    
    In this section, we provide the euclidean gradients for each covariance matrix plug-in applied to the Frobenius norm.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with \ac{SCM} / \ac{PO} plug-in
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} = - 4 \left( \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) + \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ \mathbf{Z}) \right)^H 
        \label{grad_Frob_unstruct}
    \end{align}
    \end{proposition}
    
    More details about the calculations can be found in Appendix \ref{app_RGD_Frob_unstruct}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with shrinking to identity regularization
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} &= - 4 \left(\beta \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) + \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ \mathbf{Y} ) \right)^H
        \label{grad_Frob_shrink}
    \end{align}
    \end{proposition}
    
    Further details about the calculations can be found in Appendix \ref{app_RGD_Frob_shrink}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with tapered covariance matrix
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} &= - 4 \left( \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ (\mathbf{U}^T \circ \mathbf{V}^H) ) \right. \notag \\
        &+\left. \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ (\mathbf{T} \circ \mathbf{Z})) \right)^H 
        \label{grad_Frob_tap}
    \end{align}
    \end{proposition}
    
    Details about the calculations can be found in Appendix \ref{app_RGD_Frob_tap}.
    
    \begin{algorithm}[H]
    \caption{Riemannian gradient descent algorithm for Frobenius norm with an unstructured plug-in}
        \begin{algorithmic}
            \State \textbf{Input}: Objective function \( f \) (eq. \ref{cost_fct_bloc_Frob}), starting point \( \mathbf{\bar{w}}_{\theta}^{(0)} \)
            \Repeat
                \State Compute Euclidean gradient with (\ref{grad_Frob_unstruct})
                \State Compute Riemannian gradient with (\ref{inner_product})
                \State Set direction \( \mathbf{\xi}^{(t)} = - \alpha \eta^{(t)} \)
                \State Update \( \mathbf{\bar{w}}^{(t)} = \mathcal{R}_{\mathbf{w}^{(t)}}(\mathbf{\xi}^{(t)}) \)
            \Until{convergence}
            \State \textbf{Output}: \( \hat{\mathbf{w}}_{\theta} = \mathbf{\bar{w}}_{\text{end}} \in \mathbb{T}_k \)
        \end{algorithmic}
    \end{algorithm}

% MM frob
    
    \begin{proposition}
    Majorization function for the Frobenius norm along with the \ac{SCM} / \ac{PO} plug-in 
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) = - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[(\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} +  (\mathbf{B} \circ \mathbf{Z}) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
    \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_Frob_unstruct}.
    
    \begin{proposition}
    Majorization function for the Frobenius norm along with the shrinking to identity regularization
    \begin{align}
        g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) = - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[\beta(\mathbf{A} \circ \mathbf{V} ) \mathbf{w}_{\theta} +  (\mathbf{B} \circ \mathbf{Y}) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
    \end{align}
    \end{proposition}
    More details can be found in Appendix \ref{app_MM_Frob_shrink}.
    
    \begin{proposition}
        Majorization function for the Frobenius norm along with the covariance matrix tapering regularization
        \begin{align}
            g(\mathbf{\Bar{w}}_{\theta} | \mathbf{\Bar{w}}_{\theta}^{(t)}) &= - \text{Re}\left(\mathbf{\Bar{w}}_{\theta}^H  4 \left[(\mathbf{A} \circ (\mathbf{U} \circ \mathbf{V}) ) \mathbf{w}_{\theta} \right. \right. \notag \\
            &\left. \left. +  (\mathbf{B} \circ (\mathbf{T} \circ \mathbf{Z})) \mathbf{\Bar{w}}_{\theta}^{(t)} \right] \right)
        \end{align}
    \end{proposition}
    Further details can be found in Appendix \ref{app_MM_Frob_tap}.
    
    \noindent
    Then the minimization problem can be solved using Lemma \ref{lemma2}.
    
    \begin{algorithm}[H]
    \caption{\\ac{MM} for Frobenius norm with an unstructured plug-in}
    \begin{algorithmic}[1]
        \State \textbf{Input}: $\mathbf{\tilde{\Sigma}} \in \mathbb{C}^l$, $\mathbf{w}_{\theta}^{(1)} \in \mathbb{T}_l$
        \State Compute  $\mathbf{M} = \mathbf{A} \circ \mathbf{V}$ 
        \State Compute  $\mathbf{N} = \mathbf{B} \circ \mathbf{Z}$ 
        \Repeat
            \State Compute $\mathbf{\bar{w}}^{(t)} = \mathbf{M} + \mathbf{N} w^{(t)}$
            \State Update of $ \mathbf{\bar{w}}_{\theta}^{(t)} = \phi_{\mathbb{T}}\{ \mathbf{\bar{w}}_{\theta}^{(t)} \} $ 
            \State $t = t + 1$
        \Until{convergence}
        \State \textbf{Output}: $\hat{\mathbf{w}}_{\theta} = \mathbf{\bar{w}}^{(\text{end})} \in \mathbb{T}_k$
    \end{algorithmic}
    \end{algorithm}

% RGD Frob
\paragraph{Riemannian optimization}

In this section, we provide the euclidean gradients for each covariance matrix plug-in applied to the Frobenius norm.

    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with \ac{SCM} / \ac{PO} plug-in
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} = - 4 \left( \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) + \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ \mathbf{Z}) \right)^H 
        \label{grad_Frob_unstruct}
    \end{align}
    \end{proposition}
    
    More details about the calculations can be found in Appendix \ref{app_RGD_Frob_unstruct}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with shrinking to identity regularization
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} &= - 4 \left(\beta \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ \mathbf{V}^H ) + \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ \mathbf{Y} ) \right)^H
        \label{grad_Frob_shrink}
    \end{align}
    \end{proposition}
    
    Further details about the calculations can be found in Appendix \ref{app_RGD_Frob_shrink}.
    
    \begin{proposition}
    Euclidean gradient for \ac{KL} divergence with tapered covariance matrix
    \begin{align}
        \textit{grad} f^{\text{LS}}_{\mathbf{\widetilde{\Sigma}}} &= - 4 \left( \mathbf{w}_{\theta}^H (\mathbf{A}^T \circ (\mathbf{U}^T \circ \mathbf{V}^H) ) \right. \notag \\
        &+\left. \mathbf{\Bar{w}}_{\theta}^H (\mathbf{B} \circ (\mathbf{T} \circ \mathbf{Z})) \right)^H 
        \label{grad_Frob_tap}
    \end{align}
    \end{proposition}
    
    Details about the calculations can be found in Appendix \ref{app_RGD_Frob_tap}.
    
    \begin{algorithm}[H]
    \caption{Riemannian gradient descent algorithm for Frobenius norm with an unstructured plug-in}
        \begin{algorithmic}
            \State \textbf{Input}: Objective function \( f \) (eq. \ref{cost_fct_bloc_Frob}), starting point \( \mathbf{\bar{w}}_{\theta}^{(0)} \)
            \Repeat
                \State Compute Euclidean gradient with (\ref{grad_Frob_unstruct})
                \State Compute Riemannian gradient with (\ref{inner_product})
                \State Set direction \( \mathbf{\xi}^{(t)} = - \alpha \eta^{(t)} \)
                \State Update \( \mathbf{\bar{w}}^{(t)} = \mathcal{R}_{\mathbf{w}^{(t)}}(\mathbf{\xi}^{(t)}) \)
            \Until{convergence}
            \State \textbf{Output}: \( \hat{\mathbf{w}}_{\theta} = \mathbf{\bar{w}}_{\text{end}} \in \mathbb{T}_k \)
        \end{algorithmic}
    \end{algorithm}


